Gauntlet: Finding Bugs in Compilers for Programmable Packet Processing

Programmable packet-processing devices such as programmable switches and network interface cards are becoming mainstream. These devices are configured in a domain-specific language such as P4, using a compiler to translate packet-processing programs into instructions for different targets. As networks with programmable devices become widespread, it is critical that these compilers be dependable. This paper considers the problem of finding bugs in compilers for packet processing in the context of P4-16. We introduce domain-specific techniques to induce both abnormal termination of the compiler (crash bugs) and miscompilation (semantic bugs). We apply these techniques to (1) the open-source P4 compiler (P4C) infrastructure, which serves as a common base for different P4 back ends; (2) the P4 back end for the P4 reference software switch; and (3) the P4 back end for the Barefoot Tofino switch. Across the 3 platforms, over 8 months of bug finding, our tool Gauntlet detected 96 new and distinct bugs (62 crash and 34 semantic), which we confirmed with the respective compiler developers. 54 have been fixed (31 crash and 23 semantic); the remaining have been assigned to a developer. Our bug-finding efforts also led to 6 P4 specification changes. We have open sourced Gauntlet at p4gauntlet.github.io and it now runs within P4C's continuous integration pipeline.

==> Makefile <==
# Put user-specific changes in your own Makefile.user.
# Make will silently continue if that file does not exist.
-include Makefile.user

TARGET   = main
TARGET_BIB   = biblio

STYFILES = $(wildcard *.sty) $(wildcard *.cls)

PSTOPDF ?= pstopdf

.SUFFIXES:	.plot .eps .pdf

all: $(TARGET).pdf

draft: $(TARGET).pdf
	mkdir -p drafts
	cp $(TARGET).pdf drafts/draft-$(shell date "+%Y-%m-%d")-$(shell cat *.tex | shasum | head -c 8).pdf

html: $(TARGET).html

# used to launch editor that works with synctex etc
# see: https://github.com/mhinz/neovim-remote
editor:
	NVIM_LISTEN_ADDRESS=/tmp/nvimsocket nvim

#copy over biblio file from craig's related work file
EXTRA_DEPS := \
	 biblio.bib

OUTSIDE_BIB := ../biblio.bib
#this rule does nothing on purpose so this works on systems without the outside bib
# on systems with such a file, it copies it over
$(OUTSIDE_BIB):
	# bib creation no-op
biblio.bib: $(OUTSIDE_BIB)
	if [ -f $(OUTSIDE_BIB) ]; then cp $(OUTSIDE_BIB) . ; fi

$(TARGET).html: ${PDF_FIGURES} $(TARGET).bbl $(wildcard *.tex) $(STYFILES)  $(EXTRA_DEPS)
	htlatex $(TARGET).tex
	htlatex $(TARGET).tex

$(TARGET).pdf: ${PDF_FIGURES} $(TARGET).bbl $(wildcard *.tex) $(STYFILES)  $(EXTRA_DEPS)
	pdflatex $(TARGET).tex
	pdflatex $(TARGET).tex

$(TARGET).aux: $(TARGET).tex $(wildcard *.tex)
	pdflatex $(TARGET)

$(TARGET).bbl: $(TARGET_BIB).bib $(TARGET).aux
	pdflatex $(TARGET).tex
	bibtex $(TARGET)

tags: TAGS
.PHONY: tags TAGS html
TAGS:
	etags `latex-process-inputs --list usenix.tex`

clean:
	rm -f $(TARGET).pdf
	rm -f $(TARGET).log
	rm -f $(TARGET).blg
	rm -f $(TARGET).aux
	rm -f $(TARGET).bbl
	rm -f $(TARGET).dvi
	rm -f $(TARGET).out
	rm -f $(TARGET).toc
	rm -f $(TARGET).html $(TARGET).css $(TARGET).4ct $(TARGET).4tc \
		$(TARGET).xref $(TARGET).idv $(TARGET).lg $(TARGET).tmp \
		$(TARGET)*.html


==> figures/techniques_design.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{./figures/p4_background.pdf}
    \caption{An example P4 compilation model.}
    \label{fig:p4_background}
\end{figure}

\begin{figure*}[tb]
    \begin{minipage}[t]{0.49\linewidth}
    \centering
        \includegraphics[width=1\linewidth]{./figures/translation_validation.pdf}
        \caption{Translation validation.\label{fig:workflow_validation}}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.498\linewidth}
    \centering
        \includegraphics[width=1\linewidth]{./figures/semantics_guided_fuzzing.pdf}
        \caption{Symbolic execution.\label{fig:workflow_fuzzing}}
    \end{minipage}
    \hfill
\end{figure*}


